Wait-Only Broadcast Protocols are Easier to Verify

We study networks of processes that all execute the same finite-state protocol and communicate via broadcasts. We are interested in two problems with a parameterized number of processes: the synchronization problem which asks whether there is an execution which puts all processes on a given state; and the repeated coverability problem which asks if there is an infinite execution where a given transition is taken infinitely often. Since both problems are undecidable in the general case, we investigate those problems when the protocol is Wait-Only, i.e., it has no state from which a process can both broadcast and receive messages. We establish that the synchronization problem becomes Ackermann-complete, and the repeated coverability problem is in EXPSPACE, and PSPACE-hard.

==> app-sec-rep-cover-swo.tex <==
\section{Proof of \cref{sec:rep-cover-swo}}
\begin{proof}[Proof of \cref{lemma:rep-cover-swo-rbn}]
	Let $\PP = (Q, \Sigma, \qinit, T)$ be a Single-Wait-Only protocol and $t_f = (q, \alpha, q') \in T$ be a transition.
	Consider an infinite execution $ C_0 \trans C_1 \trans C_2 \trans\cdots$ and a process $\aproc \in [1, ||C_0||]$ such that for all $i \in \nat$, there exists $j > i$ with $(C_j(\aproc),\alpha, C_{j+1}(\aproc) ) = t$. Then $C_0 \transRBN C_1 \transRBN C_2\transRBN \cdots$. 
	
	Now consider the other direction: assume there exists an infinite execution $\rho =  C_0 \transRBN C_1 \transRBN C_2 \transRBN\cdots$ and a process $\aproc_t \in [1, ||C_0||]$ such that for all $i \in \nat$, there exists $j > i$ with $(C_j(\aproc_t),\alpha, C_{j+1}(\aproc_t) ) = t_f$. 
	
	We build an execution $C'_0 \trans C'_1 \trans C'_2 \trans\cdots$ such that for all $i \in \nat$, for all $\aproc \in [1, ||C'_0||]$ which is \emph{not} dead from $i$:
	\begin{enumerate}[(A)]
		\item if $C_i(\aproc)\in Q_A$, $C'_i(\aproc)= C_i(\aproc)$;
		\item if $C_i(\aproc) \in Q_W$ and $\nextactionindex{\rho, i, \aproc} = \omega$, and $\aproc$ is immortal, then there exists $j \geq i$, such that $C'_i(\aproc) = C_j(\aproc)$;
		\item if $C_i(\aproc) \in Q_W$ and $\nextactionindex{\rho, i, \aproc}  \in \nat$, then $C'_i(\aproc)\in \set{C_i(\aproc), \dots, C_{\nextactionindex{\rho, i, \aproc}}(\aproc)}$.
	\end{enumerate}
	We build the execution by induction on $i \in \nat$. For $i = 0$, as $C'_0 = C_0$, the property trivially holds. Let $i \in \nat$ and assume we have built  $C'_0 \trans C'_1 \trans C'_2 \trans\cdots \trans C'_i$ with $C'_i$ respecting the property. 
	Denote $C_i \transRBNup{\aproc, t} C_{i+1}$ with $t = (q, !!a, q') \in T$. We define $C'_{i+1}$ as:
	$C'_{i+1}(\aproc) = q'$, and for all $\aproc'$:
	\begin{itemize}
		\item if there exists $p'$ such that $(C'_{i}(\aproc'), ?a, p') \in T$, then $C'_{i+1}(\aproc') = p'$;
		\item otherwise, $C'_{i+1}(\aproc')= C'_i(\aproc')$.
	\end{itemize}
	We first prove that $C'_i \transup{\aproc, t } C'_{i+1}$. From the definition of $C'_{i+1}$, we only have to prove that $C'_i(\aproc) = q$. This directly follows from (A) on $C'_i$ as $q \in Q_A$. 
	We now prove that (A),(B) and (C) hold for $C'_{i+1}$.
	
	\emph{Proof of (A):} let $\aproc'$ such that $C_{i+1}(\aproc') \in Q_A$; then we are in one of the following cases:
	\begin{itemize}
		\item $\aproc' = \aproc$ and $C_{i+1}(\aproc) = q' \in Q_A$, in that case, $C'_{i+1}(\aproc) = C_{i+1}(\aproc) = q'$;
		\item $\aproc' \neq \aproc$ and $C_{i+1}(\aproc') = C_i(\aproc) $ and $C_i(\aproc) = C'_i(\aproc)$ by induction hypothesis with (A). By construction, we get that $C'_{i+1}(\aproc') = C'_i(\aproc) = C_i(\aproc) = C_{i+1}(\aproc)$;
		\item $\aproc' \neq \aproc$ and $(C'_i(\aproc'), ?a, C'_{i+1}(\aproc'))\in T$. 
		As $C_{i+1}(\aproc') \in Q_A$ and $C_{i}(\aproc')\in Q_W$, we are in case (C) and $\nextactionindex{\rho, i, \aproc'}= i+1$. Hence, by induction hypothesis, $C'_i(\aproc') \in \set{C_i(\aproc'), C_{i+1}(\aproc')}$. If $C'_i(\aproc') = C_i(\aproc')$, then as $\PP$ is Single-Wait-Only, there is a unique $p = C_{i+1}(\aproc')$ such that $(C'_i(\aproc'), ?a, p) \in T$. Hence, by construction, $C_{i+1}'(\aproc') = C_{i+1}(\aproc')$;
		If $C'_i(\aproc') = C_{i+1}(\aproc')$, then by construction $C'_{i+1}(\aproc') = C'_i(\aproc')$ as $C'_{i}(\aproc') \in Q_A$, hence (A) holds.
	\end{itemize}
	
	
	\emph{Proof of (B):} let $\aproc'$ a process such that $C_{i+1}(\aproc') \in Q_W$ such that $\nextactionindex{\rho, i+1, \aproc} = \omega$; then we are in one of the following cases:
	\begin{itemize}
		\item if $C_i(\aproc') \in Q_W$, then  $\nextactionindex{\rho, i, \aproc'} = \omega$ and by induction hypothesis with (B), there exists $j \leq i$ such that $C'_i(\aproc') = C_j(\aproc')$. Either (i) $(C'_i(\aproc'), ?a ,C'_{i+1}(\aproc')) \in T$ or (ii) $C'_{i+1}(\aproc') = C'_i(\aproc')$. In case (i), as $\aproc'$ is immortal, there must exists $k > j$ such that $C_{k}(\aproc') = C'_{i+1}(\aproc')$: Indeed, since $\aproc'$ moves state at one point after $C_j$, and since $\PP$ is Single-Wait-Only, the only ougoing transition from $C_j(\aproc')$ is $(C_{j}(\aproc'), ?a ,C'_{i+1}(\aproc'))$, which concludes this case. 
		In case (ii), $C'_{i+1}(\aproc') = C'_i(\aproc') = C_j(\aproc')$. The only problematic case would be if $j = i$ and $C_{i+1}(\aproc') \neq C_i(\aproc')$: in that case, $(C_i(\aproc') , ?a , C_{i+1}(\aproc') ) \in T$ and $C'_i(\aproc') = C_i(\aproc')$ which contradicts the construction of $C'_{i+1}$;
		
		\item if $C_i(\aproc') \in Q_A$, then $\aproc' = \aproc$, and by induction hypothesis $C'_i(\aproc) = C_i(\aproc)$, and $C'_{i+1}(\aproc) = q' = C_{i+1}(\aproc)$, which concludes this case;
		
	\end{itemize}
	
	
	\emph{Proof of (C):}  let $\aproc'$ be a process such that $C_{i+1}(\aproc') \in Q_W$ such that $\nextactionindex{\rho, i+1, \aproc'}  = n$; then we are in one of the following cases:
	\begin{itemize}
		\item $(C_i(\aproc'), ?a, C_{i+1}(\aproc')) \in T$. Then $C_i(\aproc')\in Q_W$ and $\nextactionindex{\rho, i, \aproc'}  = n$, hence by induction hypothesis with (C) $C'_i(\aproc') \in \set{C_i(\aproc'), \dots C_n(\aproc')}$. If $C'_i(\aproc') = C_i(\aproc')$ then as $\PP$ is Single-Wait-Only, there exists a unique $p \in Q$ such that $(C'_i(\aproc'), ?a, p)\in T$ and $p = C_{i+1}(\aproc')$. Hence, by construction, $C'_{i+1}(\aproc') = p$. Otherwise, $C'_i(\aproc') \in \set{C_{i+1}(\aproc'), \dots C_n(\aproc')}$, then if $C'_{i+1}(\aproc') = C'_{i}(\aproc')$, this case is done. Othserwise, $(C'_i(\aproc'), ?a, C'_{i+1}(\aproc')) \in T$. As $\PP$ is Single-Wait-Only, this is the unique outgoing transition from $C'_i(\aproc')$, hence, as $C'_i(\aproc') \in Q_W$, $C'_i(\aproc') \neq C_n(\aproc') \in Q_W$ and so $C'_{i+1}(\aproc') \in \set{C_{i+2}(\aproc'), \dots, C_n(\aproc')}$, which concludes this case; 
		\item $C_{i+1}(\aproc') = C_i(\aproc') \in Q_W$. Then, $\nextactionindex{\rho, i, \aproc'}  = n$, hence by induction hypothesis with (C) $C'_i(\aproc') \in \set{C_i(\aproc'), \dots C_n(\aproc')}$. 
		If $C'_i(\aproc') = C_i(\aproc')$, then there is no outgoing transition labeled with $?a$ from $C'_i(\aproc')$ (as $C_i(\aproc')= C_{i+1}(\aproc')$) and so by construction $C'_{i+1}(\aproc')$ which proves (C).
		If $C'_i(\aproc) \in \set{C_{i+1}(\aproc), \dots, C_n(\aproc)}$, then if $C'_{i+1}(\aproc) = C'_i(\aproc)$, proof of (C) is done. Otherwise, $(C'_i(\aproc'), ?a, C'_{i+1}(\aproc')) \in T$. As $\PP$ is Single-Wait-Only, this is the unique outgoing transition from $C'_i(\aproc')$, hence, as $C'_i(\aproc') \in Q_W$, $C'_i(\aproc') \neq C_n(\aproc') \in Q_W$ and so  $C'_{i+1} \in \set{C_{i+2}(\aproc), \dots,  C_n(\aproc)}$.
		\item $\aproc' = \aproc$ and $C_{i+1}(\aproc') = q' \in Q_W$, and by cosntruction $C'_{i+1}(\aproc) = q'$. 
		
		
	\end{itemize}
	
	Hence, we proved the existence of an infinite execution $C'_0 \trans C'_1 \trans C'_2 \trans\cdots$ respecting conditions (A), (B) and (C).
	To conclude the proof we distinguish between two cases:
	\begin{itemize}
		\item case with $t_f = (q, !!a, q')$ for some $q, q' \in Q$ and $a \in \Sigma$. Then, for all $i \in \nat$, there exists $j \geq i$ such that $C_j \transRBNup{\aproc_t, t_f} C_{j+1}$. We proved that $C'_j \transup{\aproc_t, t_f} C'_{j+1}$, which concludes this case.
		\item case with $t_f = (q, ?a, q')$  for some $q, q' \in Q$ and $a \in \Sigma$. Then, for all $i \in \nat$, there exists $j \geq i$ such that $(C_j(\aproc_t), ?a , C_{j+1}(\aproc_t)) = t_f$. If $\nextactionindex{\rho, j, \aproc_t} = \omega$, then, as $\aproc_t$ is immortal, using (B) and the fact that $t$ is the only outgoing transition from $q$, we get that there exists $k \geq j$ such that $(C'_k(\aproc_t), ?a , C'_{k+1}(\aproc_t)) = t_f$.
		If $\nextactionindex{\rho, j, \aproc_t} \in \nat$, using (C) and the fact that $t$ is the only outgoing transition from $q$, we get that there exists $j \leq k \leq \nextactionindex{\rho, j, \aproc_t} $ such that $(C'_k(\aproc_t), ?a , C'_{k+1}(\aproc_t)) = t_f$.
	\end{itemize}
	
	
	
\end{proof}



==> app-sec-synchro-swo-hardness.tex <==
\subsection{Proofs of \cref{subsec:synchro-swo-hardness}}

\begin{lemma}
	If there exists a world $w \in \bigcap_{1  \leq i \leq n } L(\mathcal{A}_i)$, then there exists 
	$C_0 \trans^\ast C_f$ such that $C_0 \in \mathcal{I}$ and for all $\aproc \in [1, ||C_f||]$, $C_f(\aproc) = q_f$.  
\end{lemma}
\begin{proof}
	Denote $w = a^1 \dots a^k \in \bigcap_{1  \leq i \leq n } L(\mathcal{A}_i)$, and consider $C_0$ the initial configuration with $n+1$ processes in $\qinit$.
	Consider the following sequence of events:
	$C_0 \transup{n+1, (\qinit, !! \$, q_1)} C_1 \transup{1, (\qinit, !!1, q_1^0)} \cdots \transup{n, (\qinit, !!n, q_n^0)} C_{n+1}$; $C_{n+1}$ is such that $C_{n+1}(i) = q_i^0$ for all $1 \leq i \leq n$ and $C_{n+1}(n+1) = q_{n+1}$.
	
	
	For all $1 \leq j \leq k$ and for all $1\leq i \leq n$, we denote $q_i^j$ the sate $\Delta_i^\ast(\qinit, a^1\cdots a^j)$.
	
	From $C_{n+1}$ consider the following chain of events: 
	$C_{n+1} \transup{1, (q_0^1 , !!\$, (q_0^1, a^1, 1))} C_{n+2} \transup{2, (q_0^2, !!\$, (q_0^2, a^1, 1))} \cdots \transup{n, (q_0^n , !!\$, (q_0^n, a^1, n))} C_{2n+1} \transup{n+1, (q_{n+1}, !! a^1, q_1^{a^1})} C_{2n+2} \transup{1, ( (q_1^1, a,2), !!a_1^1, q_1^1)} \cdots  \transup{n, ( (q_1^n, a^1,2), !!a^1_n, q_n^1)} C_{3n+2}$.
	$C_{3n+2}$ is such that $C_{3n+2}(i) = q_i^1$ for all $1 \leq i \leq n$ and $C_{3n+2}(n+1) = q_{n+1}$.
	%	\transup{n+1, (q_{n+1}, !!a^1, q_1^{a^1})} C_{n+2}\transup{1, (q_0^1n+1}, !!a^1, q_1^{a^1})} $
We can continue the execution in the same way until reaching configuration $C_{n(2k+1) + k+1}$ such that $C_{n(2k+1) + k+1}(i) = q_i^k = q_i^f$ for all $1 \leq i \leq n$ and $C_{n(2k+1) + k+1}(n+1) = q_{n+1}$.
To end the execution, consider the following sequence of configurations: 
$C_{n(2k+1) + k+1} \transup{1, (q^1_f, !! \$ ,p_1)} \transup{2, (q^2_f, !! \$ ,p_1)} \cdots $ \ $ \transup{n, (q^n_f, !! \$ ,p_1)} C_{n(2k+2)+ k +1}\transup{n+1, (q_{n+1}, !! \textsf{end}, q_{n+2})} C_{n(2k+2)+ k +2} \transup{1, (p_2, !! \textsf{end} ,p_3)} \transup{2, (p_2, !! \textsf{end} ,p_3)} \cdots$\  $ \transup{n, (p_2, !! \textsf{end} ,p_3)} \transup{1, (p_3, !! \$ ,q_f)} \transup{2, (p_3, !! \$ ,q_f)} \cdots$ \ $  \transup{n, (p_3, !! \$ ,q_f)} C_{n(2k+4) + k+2}$. Observe that $C_{n(2k+4) + k+2}$ is such that$C_{n(2k+4) + k+2}(i) = q_f$ for all $1 \leq i \leq n+1$.

\end{proof}


\begin{lemma}
Let $C_0 \trans^\ast C_f$ such that $C_0 \in \mathcal{I}$ and for all $\aproc \in [1, ||C_f||]$, $C_f(\aproc) = q_f$. Then there exists a world $w \in \bigcap_{1  \leq i \leq n } L(\mathcal{A}_i)$.
\end{lemma}
\begin{proof}
Let $C_0 \trans^\ast C_f$ such that $C_0 \in \mathcal{I}$ and for all $\aproc \in [1, ||C_f||]$, $C_f(\aproc) = q_f$. We start by proving different claims.

\begin{claim}
	There is exactly one process $\aproc$ taking the transition $(q_{n+1}, !!\textsf{end}, q_{n+2})$ between $C_0$ and $C_f$.
\end{claim}
\begin{proof}
	There is at least one as otherwise $q_f$ is not even coverable. Assume there is two processes $\aproc,\aproc'$ taking the transition $(q_{n+1}, !!\textsf{end}, q_{n+2})$. Assume $\aproc$ takes it first, then when $\aproc'$ broadcasts $\textsf{end}$, $\aproc$ receives it and leaves $q_{n+2}$ anymore. From this moment, $\aproc$ and $\aproc'$ cannot be reunited again except in $\textsf{err}$, which contradicts the fact that $C_f(\aproc) =C_f(\aproc') = q_f$. 
\end{proof}

We denote $j_0$ the index such that $C_{j_0} \transup{\aproc, (q_{n+1}, !!\textsf{end}, q_{n+2})} C_{j_0 +1}$.

\begin{claim}
	There are exactly $n$ processes taking the transition $(p_2, !! \textsf{end}, p_3)$ between $C_0$ and $C_f$.
\end{claim}
\begin{proof}
	Observe that by construction of $\PP$, there is no broadcasts of $\textsf{end}$ with transition $(p_2, !!\textsf{end} , p_3)$ possible before index $j_0$, as $(p_1, ?\textsf{end}, p_2)$ and $\aproc$ is the unique process to take transition $(p_2, !! \textsf{end}, p_3)$ from the previous claim. 
	
	Hence, the first time transition $(p_2, !! \textsf{end}, p_3)$ is taken happens after $j_0$. Observe that if there is less than $n$ broadcasts of $\textsf{end}$, then $C_f(\aproc) \in \set{q_{n+2}, \dots ,q_{2n+1}}$ (and so $C_f(\aproc) \neq q_f$), and if there is more than $n$ broadcasts of $\textsf{end}$, then $C_f(\aproc)  = \textsf{err}  \neq q_f$.
	Hence, there is exacty $n$ processes taking transition $(p_2, !! \textsf{end}, p_3)$.
\end{proof}

\begin{claim}
	For all $1 \leq i \leq n$, there is exactly one process $\aproc_i$ taking the transition $(\qinit, !!i, q_0^i)$ between $C_0$ and $C_f$.
\end{claim}
\begin{proof}
	Let $1 \leq i \leq n$, there is at least one process taking the transition $(\qinit, !!i, q_0^i)$, as otherwise $\aproc$ never receives message $i$ which contradicts the fact that $C_{j_0}(\aproc) = q_{n+1}$. As this reasoning holds for all $1 \leq i\leq n$, if there is more than one process  taking a transition $(\qinit, !!i, q_0^i)$, then there will be more than $n$ processes taking the transition $(p_2, !! \textsf{end}, p_3)$ which contradicts the previous claim. Hence there is exactly one such process.
\end{proof}

From the three previous lemma we get that $||C_0|| = n+1$ and there exists $j_1$ such that $C_{j_1-1} \transup{\aproc_n, (\qinit, !! n, q_0^n)} C_{j_1}$ and $C_{j_1}(\aproc) = q_{n+1}$, and $C_{j_1}(\aproc_i) \in \set{q_0^i, (q_0^i, a, 1) \mid a \in \Sigma}$ for all $1 \leq i\leq n$.

We denote $k_0, \dots, k_N$ the set of indices such that $C_{k_\ell} \transup{\aproc, (q, !!m ,q')} C_{k_\ell+1}$ with $(q, !!m, q') \in T$, for all $0 \leq \ell \leq N$, i.e. the set of indices from which $\aproc$ broadcasts a message. Observe that by construction of the VASS, $k_0 \geq j_1$.

We now prove the following claim.
\begin{claim}
	For all $0 \leq \ell < N$ such that $C_{k_\ell} \transup{\aproc, (q, !!m ,q')} C_{k_\ell+1}$, and for all $1 \leq i \leq n$, it holds that $(C_{k_\ell}(\aproc_i), ?m, C_{k_\ell+1}(\aproc_i)) \in T$. 
\end{claim}
\begin{proof}
	%We start by proving the claim for $\ell = N$, and then we prove it by induction for all $0 \leq \ell < N$. 
	%
	%When $\ell = N$, $C_{k_\ell} \transup{\aproc, (q_{n+1}, !!\textsf{end} ,q_{n+2})} C_{k_\ell+1}$ as $k_N$ is the last moment where $\aproc$ broadcasts a message and $C_f(\aproc) = q_f$. 
	%If there exists $1 \leq i \leq n$, such that $\aproc_i$ does not receive the message $\textsf{end}$, then 
	
	We prove the claim by induction on $0 \leq \ell < N$. Observe that, in any cases, as $\ell \neq N$, there is an index $k_{\ell+1}$ such that $C_{k_{\ell+1}}(\aproc) = q_{n+1}$, hence for all $0 \leq \ell < N$, $C_{k_\ell} \transup{\aproc, (q_{n+1}, !!a^\ell ,q_{1}^{a^\ell})} C_{k_\ell+1}$ with $a^{\ell}\in \Sigma$ for all $0 \leq \ell < N$. 
	
	For $\ell = 0$, as $k_0$ is the first index from which $\aproc$ broadcasts and $\aproc$ is the only process who can broadcast a message $a \in \Sigma$, $C_{k_0}(\aproc_i) \in \set{q_0^i, (q_0^i, a, 1) \mid a \in \Sigma}$ for all $1 \leq i\leq n$. If there exists a process $\aproc_i$ which does not receive the message, then $C_{k_0 + 1}(\aproc_i) \in \set{q_0^i, (q_0^i, a, 1) \mid a \in \Sigma}$. By definition, $\aproc$ does not broadcast anything between $C_{k_0 + 1}$ and $C_{k_1}$. Hence, $\aproc_i$ does not broadcast any message (except $\$$) between $C_{k_0 +1}$ and $C_{k_1}$. As it is the only process in $\PP_{\mathcal{A}_i}$, $C_{k_1}(\aproc) \in \set{q_{1}^{a^0}, q_2^{a^0}, \dots q_i^{a^0}}$, which contradicts the fact that $\aproc$ broadcasts from $C_{k_1}$. As a consequence, all processes receive the message. 
	
	Let $0 \leq \ell <N-1$. We suppose that the property holds for $\ell$, hence if $C_{k_\ell} \transup{\aproc, (q_{n+1}, !!a^\ell ,q_{1}^{a^\ell})} C_{k_\ell+1}$, then $C_{k_{\ell }+ 1}(\aproc_i)  = (q^\ell_i, a^\ell, 2) $ for some $q^\ell_i \in Q_i$ for all $1 \leq i \leq n$. Let $1 \leq i \leq n$, $C_{k_{\ell +1}}(\aproc) = q_{n+1}$ and $\aproc_i$ is the only process able to broadcast $a^\ell_i$, there is an index where it does so and the message is received by $\aproc$ (as otherwise, $\aproc$ never reaches $q_{n+1}$ again). As $\aproc$ does not broadcast anything between $C_{k_\ell + 1}$ and $C_{k_{\ell+1 }}$, $C_{k_{\ell +1}}(\aproc_i) \in \set{q^\ell_i, (q^\ell_i, a, 1) \mid a \in \Sigma}$.
	If there exists a process $\aproc_i$ which does not receive the message, then $C_{k_{\ell + 1} + 1}(\aproc_i) \in \set{q_i^\ell, (q_i^\ell, a, 1) \mid a \in \Sigma}$. By definition, $\aproc$ does not broadcast anything between $C_{k_{\ell +1} + 1}$ and $C_{k_{\ell+2}}$. Hence, $\aproc_i$ does not broadcast any message (except $\$$) between $C_{k_{\ell +1} +1}$ and $C_{k_{\ell +2}}$. As it is the only process in $\PP_{\mathcal{A}_i}$, $C_{k_{\ell +2}}(\aproc) \in \set{q_{1}^{a^\ell}, q_2^{a^\ell}, \dots q_i^{a^\ell}}$, which contradicts the fact that $\aproc$ broadcasts from $C_{k_{\ell +2}}$. As a consequence, all processes receive the message. 
	
	
\end{proof}

%Observe that $i_N = j_0$. 
%We justify by induction that for all $1 \leq \ell \leq N$, there exists a world $w = a^1 \cdots a^{K_\ell}$ such that for all $1 \leq j \leq n$, $C_{i_\ell +1}(\aproc_j) \in \set{q^j, (q^j, a, 1) \mid q^j\in Q_j, a \in \Sigma \textrm{ and }q^j= \Delta^\ast(q_0^j ,w )} \cup \set{p_1 \textrm{ if } \ell = N}$.
%
%For $\ell = 0$, $i_0$ is the first index from which $\aproc $ leave $q_{n+1}$, hence no message $a \in \Sigma$ has been broadcast yet, and hence, $C_{i_0}(\aproc_j) \in \set{q_0^j, (q_0^j, a, 1) \mid a \in \Sigma}$ for all $1 \leq j\leq n$. As $\Delta^\ast (q_0^j, \epsilon) = q_0^j$ for all $j \in [1,n]$, we choose $w = \epsilon$. \lug{dire quelque chose sur $N = 0$ ?}
%
%Assume the property to hold for $\ell < N$, and denote $w = a^1 \cdots a^{K_\ell}$ such that for all $1 \leq j \leq n$, $C_{i_\ell +1}(\aproc_j) \in \set{q^j, (q^j, a, 1) \mid q^j\in Q_j, a \in \Sigma \textrm{ and }q^j= \Delta^\ast(q_0^j ,w )} \cup \set{p_1 \textrm{ if } \ell = N}$.

\begin{claim}
	For all $1 \leq i\leq n$, $C_{k_N}(\aproc_i) \in \set{q^f_i , p_1}$. 
\end{claim}
\begin{proof}
	Assume there exists $1 \leq i \leq n$ such that $C_{k_N}(\aproc_i) \nin \set{q^f_i , p_1}$, then, from the construction of the VASS and because $C_f(\aproc_i) = q_f$, there exists $j > k_N$ such that $C_j \transup{\aproc^j, (q, !!m, q')} C_{j+1}$ with $m \in \Sigma$. As $\aproc$ is the only process to be able to broadcast a message in $\Sigma$, $\aproc^j = \aproc$, hence this contradicts the definition of $k_N$. 
\end{proof}

Denote $a^1 \dots a^{N}$ be the sequence of messages broadcast by $\aproc$ in $\Sigma$. 
We now prove that for all $1 \leq i \leq n$, $\Delta^\ast(q_i^0, a^0 \dots a^{N}) = q_i^f$. 
To this end, let $1 \leq i \leq n$. We can denote $C_{k_{j-1}}(\aproc_i) = (q_i^{j, 1}, a^{j}, 1)$ and $C_{k_{j-1}  +1}(\aproc_i) = (q_i^{j,2}, a^{j}, 2)$ for all $1 \leq j \leq N$ as all $a^j$ are received by $\aproc_i$ from the previous claims.
By construction, no other message in $\Sigma$ is broadcast between $C_{k_j}$ and $C_{k_{j+1}}$ for all $1\leq j \leq N-1$, hence $q_i^{j,1} = q_i^{j+1,1}$. Furthermore, by the definition of $\PP_{\mathcal{A}_i}$, it holds that $(q_i^{j,1}, a^j, q_i^{j+1, 1})$. 
Futhermore, $C_{k_0}(\aproc_i) = (q_i^0, a^1, 1) $ as no message in $\Sigma$ has been broadcast yet. 
Hence together with the previous lemma: $\Delta_i^\ast(q^0_i, a^1 \cdots a^{N}) = \Delta_i^\ast(q^1_i, a^1 \cdots a^{N}) = q_i^f$
Hence, we found a world $a^1 \cdots a^{N}$ such that for all $1 \leq i \leq n$, $\Delta_i^\ast(q^0_i, a^1 \cdots a^{N}) = q^f_i$.
%\color{red}todo\color{black}
\end{proof}

==> app-sec-synchro-swo.tex <==
\section{Proofs of \cref{sec:synchro-swo}}

\input{app-sec-synchro-swo-hardness}

==> sec-rep-cover-swo-protocols.tex <==
\section{Solving the Repeated Coverability~problem with Single-Wait-Only Protocols}
\label{sec:rep-cover-swo}
In this section, we will show a reduction from Repeated Coverability problem with Single-Wait-Only Protocols to the same problem but in Reconfigurable Semantics (also called Reconfigurable Broadcast Networks). In the Reconfigurable semantics, a broadcast is received by a \emph{subset} of processes. In other words, given a protocol $\PP = (Q, \Sigma, \qinit, T)$ and two configurations $C, C'$ of the protocol $\PP$, we say that $C \transRBNup{\aproc, t} C'$ for a transition $t = (q, !!a, q') \in T$ and a process $\aproc \in [1, ||C||]$ whenever $||C|| = ||C'||$, and $C(\aproc) = q$ and $C'(\aproc) = q'$ and there exists a subset $E_r \subset [1, ||C||]$ such that $\aproc \nin E_r$ and for all $\aproc_r \in E_r$, $(C(\aproc_r), ?a, C'(\aproc_r)) \in T$ and for all $\aproc' \nin E_r$, $C(\aproc') = C'(\aproc')$. We denote $C \transRBN C'$ whenever there exists a process $\aproc $ and a transition $t$ such that $C \transRBNup{\aproc, t} C'$
Observe that in particular $C \trans C'$ implies that $C \transRBN C'$.
We extend the definition of execution to R-executions, and, given a protocol $\PP$ and a transition $t$, we denote $\RepeatedCover_{\text{R}}$ as the $\RepeatedCover$ problem that asks for an infinite \emph{R-execution} with a process taking infinitely often the transition $t$.

The following theorem holds.
\begin{theorem}[Lemma 3.4 in \cite{Fournier15Phd}, Lemma 4 in \cite{BertrandFS14}] \label{thm:rep-cover-rbn-in-ptime}
	$\RepeatedCover_{\text{R}}$ is in \textsc{PTime}.
\end{theorem}

%\color{red}todo: theorem + ref\color{black}
%\color{red}todo: denote $\RepeatedCover_{\text{RBN}}$ the problem for RBN semantics\color{black}

We prove now that the Repeated Coverability in Single-Wait-Only protocols reduces to the same problem in the Reconfigurable semantics. 
Let $\rho = C_0 \dots C_i \dots$ be an infinite sequence of configurations. We say that a process $\aproc$ is \emph{dead from $i$} whenever for all $j > i$, $C_j(\aproc) = C_i(\aproc)$. We say that a process $\aproc$ is \emph{immortal} if there is no $i\in \nat$ such that $\aproc$ is dead from $i$. 

The idea is that, from an infinite R-execution, one can construct an infinite execution where all processes must receive broadcast messages (rather than only a subset, as in the R-semantics). Intuitively, if a process receives a message that would not be received in the R-semantics, it is getting ahead. Since the protocol is Single-Wait-Only, this transition will eventually occur, as it is the only outgoing transition. If the transition does not occur, the process remains in the same state forever. In such a case, the process can be ignored, as it will never broadcast any further messages and cannot be the one taking $t_f$ infinitely often.
We get the following lemma.
\begin{lemma}\label{lemma:rep-cover-swo-rbn}
	Let $\PP$ be a Single-Wait-Only protocol and $t$ a transition of $\PP$.\  $\RepeatedCover(\PP, t)$ answers yes if and only if $\RepeatedCover_{\text{R}}(\PP, t)$ answers yes.
\end{lemma}
Using \cref{thm:rep-cover-rbn-in-ptime}, and the above lemma, we get the main theorem of this section.
\begin{theorem}
	$\RepeatedCover$ for Single-Wait-Only protocols is in \textsc{Ptime}.
\end{theorem}


%\begin{lemma}
%	Let $\PP = (Q, \Sigma, \qinit, T)$ and $t = (q, \alpha, q')\in T$. There exists an infinite RBN execution $ C_0 \transRBN C_1 \transRBN \dots$ and a process $\aproc \in [1, \nbagents{\rho}]$ such that for all $i \in \nat$, there exists $j > i$ with $(C_j(\aproc),\alpha, C_{j+1}(\aproc) ) = t$ if and only if there exists an infinite execution $ C_0 \trans C'_1 \trans C'_2 \dots$ such that for all $i \in \nat$, there exists $j > i$ with $(C_j(\aproc),\alpha, C_{j+1}(\aproc) ) = t$ 
%\end{lemma}

==> sec-synchro-swo-protocols.tex <==
	\section{Solving the \Target~problem with Single-Wait-Only Protocols}
\label{sec:synchro-swo}

\subsection{Lower bound}
\label{subsec:synchro-swo-hardness}

To prove \pspace-hardness of the \Target~problem for Single-Wait-Only protocols, we reduce the intersection non-emptiness problem for deterministic finite automata, which is known
to be \pspace-complete \cite{Kozen77}. 

Let $\mathcal{A}_1, \dots, \mathcal{A}_n$ be a list of deterministic and \emph{complete} finite automata with $\mathcal{A}_i = (\Sigma, Q_i, q_{i}^0, \set{q_i^f}, \Delta_i)$ for all $1 \leq i \leq n$. Observe that we restrict our reduction to automata with a unique accepting state, which does not change the complexity of the problem. 
We note $\Sigma^\ast$ the set of words over the finite alphabet $\Sigma$ and $\Delta^\ast_i$ the function extending $\Delta_i$ to $\Sigma^\ast$, i.e, for all $q \in Q_i$, $\Delta_i^\ast(q, \varepsilon) = q$, and for all $w \in \Sigma^\ast$ and $a \in \Sigma$, $\Delta^\ast_i(q, wa) = \Delta_i(\Delta^\ast_i(q,w), a)$. 

We build the protocol $\PP $ with set of states $Q$ displayed in \cref{fig:prot-from-auto}. For each $1 \leq i \leq n$, box $\PP_{\mathcal{A}_i}$ describes a sub protocol that we define now: $\PP_{\mathcal{A}_i} = (Q_{\mathcal{A}_i} , T_{\mathcal{A}_i} )$ where $Q_{\mathcal{A}_i}  = Q_i \cup \set{(q_i, a, 1), (q_i, a, 2) \mid q_i \in Q_i \textrm{ and } a \in \Sigma} $ and the set of transitions is displayed in \cref{fig:prot-auto}\ and defined formally here: $T_{\mathcal{A}_i}  = \set{(q_i, !!\$, (q_i,a, 1)), ((q_i, a, 2) , !!a_i, q_i ) \mid q_i \in Q_i, a \in \Sigma} \cup \set{((q_i, a, 1), ?a, (q'_i, a, 2)) \mid (q_i, a, q'_i) \in \Delta}$.

\begin{figure}
	\begin{center}
		\input{figures/prot-from-auto.tex}
	\end{center}
	\caption{Protocol $\PP$ associated to a list of autoamta $\mathcal{A}_1, \dots ,\mathcal{A}_n$.}\label{fig:prot-from-auto}
\end{figure}

\begin{figure}
	\begin{center}
		\input{figures/prot-auto.tex}
	\end{center}
	\caption{Translations of transitions $(q_i, a, q'_i)$ and $(q_i, b, q''_i)$}\label{fig:prot-auto}
\end{figure}

The reduction works as follows: one process (the leader) will receive messages $1, \dots n$, and reaches $q_{n+1}$. It will then broadcast a world: for each letter $a$ broadcasts, it waits for $n$ acknowledgments $a_1, \dots, a_n$. The acknowledgment $a_i$ is sent by the same process that broadcast message $i$, this process will evolve in $\mathcal{A}_i$: when in a state $q^i \in Q_i$, it guesses which message will be sent by the leader and goes to the corresponding state $(q^i, a, 1)$. It then receives the message $a$ sent by the leader, and reaches a state $(q'^i, a, 2)$ such that $(q^i, a, q'^^i) \in \Delta_i$, it broadcast its acknowledgment and reaches the next state $q'^i$. 
Once all processes on $q_f^1, q_f^2, \dots, q_f^n$, they all reach state $p_1$ with a broadcast of $\$$, the leader broadcasts the message $\textsf{end}$, and all other processes do the same. At the end the leader is on state $q_f$. Finally, they broadcast message $\$$ and reach $q_f$. 

As the leader needs to receive a message $i$ for every $1 \leq i \leq n$, there is at least one process simulating each automaton. 
If two processes simulate the same automaton, then once the leader broadcast one message $\textsf{end}$, at least $n+1$ messages $\textsf{end}$ will be received by the leader, and as a consequence, it will reach state $\textsf{err}$, and can never reaches $q_f$ again. For the same reason, in an execution where everyone is placed on $q_f$, there cannot be only one leader. As a consequence, each message broadcast by the leader is received by all the processes simulating the automata; as otherwise, one acknowledgment is never broadcast and the leader never reaches $q_f$.

Formal proofs are given in appendix.

\begin{theorem}
	\Target\ for Single-Wait-Only Protocols is \pspace-hard.
\end{theorem}


==> vass.tex <==
\section{Vector Addition Systems with States}

In this section, we recall the definition of Vector Addition Systems with States, as we will use it to prove some results of the paper.

A Vector Addition System with States (VASS) is a tuple $\mathcal{V} = (\Loc, \ell_0, \Counters, \Delta)$ where $\Loc$ is a finite set of locations, $\ell_0 \in \Loc$ is the \emph{initial} location, $\Counters$ is a finite set of counters and $\Delta \subseteq \Loc \times \mathbb{Z}^\Counters \times \Loc$ is a finite set of transitions. A configuration of the VASS is a tuple $(\ell, v)$ such that $\ell \in \Loc$ and $v \in \mathbb{N}^\Counters$ is a valuation over the counters. The initial configuration is $(\ell_0, \mathbf{0})$ where $\mathbf{0}(\counter) = 0$ for all $\counter \in \Counters$. Let $(\ell, v)$, $(\ell',v')$ be two configurations, and $(\ell, \delta, \ell') \in \Delta$ a transition. We say that $(\ell, v) \abconftransup{\delta} (\ell',v')$ whenever for all counters $\counter \in \Counters$, $v'(\counter) = v(\counter) + \delta(\counter) \geq 0$. We write $(\ell, v) \abconftrans (\ell', v')$ whenever there exists $(\ell, \delta, \ell') \in \Delta$ such that $(\ell, v) \abconftransup{\delta} (\ell', v')$.

A run of the VASS is a sequence of configurations starting with the initial configuration $(\ell_0, v_0), (\ell_1, v_1), \dots, (\ell_n, v_n)$ such that for all $0 \leq i <n$, it holds that $(\ell_i, v_i) \abconftransup{} (\ell_{i+1}, v_{i+1})$. 

We define the reachability problem for VASS as follows.
\begin{decproblem}
	\problemtitle{$\Reachability$~}
	\probleminput{A VASS $\mathcal{V} = (\Loc, \ell_0, \Counters, \Delta)$ and
		a  location $\ell_f \in \Loc$;} 
	\problemquestion{Is there a run from $(\ell_0, \mathbf{0})$ to $(\ell_f, \mathbf{0})$?}
\end{decproblem}

\begin{theorem}[Membership {\cite{LerouxS19}, Hardness \cite{CzerwinskiO21,Leroux21}}]\label{vass-reach-complexity}
	The Reachability problem for VASS is Ackermann-complete.
\end{theorem}

